Finding Mixed Nash Equilibria of Generative Adversarial Networks

We reconsider the training objective of Generative Adversarial Networks (GANs) from the mixed Nash Equilibria (NE) perspective. Inspired by the classical prox methods, we develop a novel algorithmic framework for GANs via an infinite-dimensional two-player game and prove rigorous convergence rates to the mixed NE, resolving the longstanding problem that no provably convergent algorithm exists for general GANs. We then propose a principled procedure to reduce our novel prox methods to simple sampling routines, leading to practically efficient algorithms. Finally, we provide experimental evidence that our approach outperforms methods that seek pure strategy equilibria, such as SGD, Adam, and RMSProp, both in speed and quality.

==> TODOs.tex <==
%
%
%
%\section{Note to myself}
%Mirror prox or Optimistic Mirror Descent differs in
%\beq
%\vx_t = \MD{\tilde{\vx}_t}{-A\vy_{t-1}}, \quad \tilde{\vx}_{t+1} = \MD{\tilde{\vx}_t}{-A\vy_{t}}. \textup{(in mirror prox, the first gradient should be $-A\tilde{\vy}_{t}$ ) }
%\eeq
%That is, the gradient is not refreshed at each iteration. Although OMD can also be applied to achieve $O(\frac{1}{T})$, I do not know if this is still true when there is an affine term. The current analysis suggests no. I might drop the OMD completely.

==> app_infMD_alg_analysis.tex <==


Classical mirror descent analysis gives the following theorems.

\begin{theorem}\label{thm:mirror_descent_Lip}
\beq
\forall \mu \in \Mcal(\Zcal), \quad \sum_{t=1}^T \ip{\mu_t - \mu}{R} \leq \frac{D_\Phi(\mu,\mu_1)}{\eta} + \frac{\eta}{2}\sum_{t=1}^T \EE\Linf{\tilde{R_t}}^2.
\eeq
\end{theorem}
\begin{proof}
We write
\begin{align}
\ip{\mu_t - \mu}{\tilde{R_t}}  &= \frac{1}{\eta} \ip{\mu_t - \mu}{\dF(\mu_t) - \dF(\mu_{t+1})} && \textup{by definition of SMD} \nn  \\
&=\frac{1}{\eta} \Big(  D_\Phi(\mu, \mu_t) + D_\Phi(\mu_t,\mu_{t+1}) - D_\Phi(\mu,\mu_{t+1})  \Big) && \textup{by \eqref{eq:three-point}} \nn\\
&= \frac{1}{\eta} \Big(  D_\Phi(\mu, \mu_t)  - D_\Phi(\mu,\mu_{t+1})  \Big)+ \frac{1}{\eta} D_{\Phi^\star}(\dF(\mu_{t+1}),\dF(\mu_{t}))  &&\textup{by \eqref{eq:duality_inf}} \nn \\
&\leq  \frac{1}{\eta} \Big(  D_\Phi(\mu, \mu_t)  - D_\Phi(\mu,\mu_{t+1})  \Big) + \frac{1}{2\eta} \Linf{ \dF(\mu_{t+1}) - \dF(\mu_{t}  )}^2 && \textup{by \eqref{eq:Fstar_smooth} \color{red}{Fix constants later}} \nn \\
&= \frac{1}{\eta} \Big(  D_\Phi(\mu, \mu_t)  - D_\Phi(\mu,\mu_{t+1})  \Big) + \frac{1}{2\eta} \Linf{ \tilde{R}_t}^2&& \textup{by definition of SMD} \nn.
\end{align}Summing up and noticing that $D_\Phi \geq 0$, we get
\beq \label{eq:hold7}
\sum_{t=1}^T\ip{\mu_t - \mu}{\tilde{R_t}} \leq \frac{D_\Phi(\mu, \mu_1) }{\eta}  + \frac{1}{2\eta} \sum_{t=1}^T\Linf{ \tilde{R}_t}^2.
\eeq
Finally, by the towering property and linearity of the expectation, we have
\begin{align}
\sum_{t=1}^T\ip{\mu_t - \mu}{R} &= \sum_{t=1}^T\ip{\mu_t - \mu}{\EE \left[\tilde{R_t}| \mu_t\right]} \nn\\
&= \EE \left[\sum_{t=1}^T\ip{\mu_t - \mu}{\tilde{R_t}} \right]. \label{eq:hold8}
\end{align}The proof is finished by taking expectation in \eqref{eq:hold7} and using \eqref{eq:hold8}.
\end{proof}


\begin{theorem}\label{thm:mirror_descent_var}
\beq
\forall \mu \in \Mcal, \quad \sum_{t=1}^T \ip{\mu_t - \mu}{R} \leq \frac{D_\Phi(\mu,\mu_1)}{\eta} + \frac{\eta}{2}\sum_{t=1}^T \EE\Linf{\tilde{R_t} - R}^2.
\eeq
\end{theorem}
\begin{proof}
We write 
\begin{align}
\ip{\mu_{t+1}   - \mu_t }{R} &= \ip{\mu_{t+1}   - \mu_t }{R- \tilde{R}_t} +  \ip{\mu_{t+1}   - \mu_t }{\tilde{R}_t}  \nn \\ 
&\leq \ip{\mu_{t+1}   - \mu_t }{\tilde{R}_t} + \Linf{R- \tilde{R}_t}  \| \mu_{t+1}   - \mu_t \|_{\Lbb^1} \nn\\
&\leq \ip{\mu_{t+1}   - \mu_t }{\tilde{R}_t}  + \frac{\eta}{2}\Linf{R- \tilde{R}_t}^2 + \frac{1}{2\eta} \| \mu_{t+1}   - \mu_t \|_{\Lbb^1}^2 \nn \\
&\leq \ip{\mu_{t+1}   - \mu_t }{\tilde{R}_t}  + \frac{\eta}{2}\Linf{R- \tilde{R}_t}^2 + \frac{1}{\eta} D_\Phi(\mu_{t+1}, \mu_t). \label{eq:hold9}
\end{align}By \eqref{eq:three-point}, for any $\mu \in \Mcal$, we have
\begin{align}
\frac{1}{\eta} \left(D_\Phi(\mu_{t+1},\mu_t) + \ip{\mu_{t+1} - \mu}{ \eta\tilde{R}_t}\right) &= \frac{1}{\eta} \Big(D_\Phi(\mu_{t+1},\mu_t) + \ip{\mu_{t+1} - \mu}{ \dF(\mu_t) - \dF(\mu_{t+1}) }\Big) \nn \\
&= \frac{1}{\eta} \Big(  D_\Phi(\mu, \mu_t) - D(\mu, \mu_{t+1})  \Big). \nn
\end{align}Continuing \eqref{eq:hold9}, we further write
\begin{align}
\ip{\mu_{t+1} }{R} &\leq \ip{\mu_t}{R}+ \ip{ \mu - \mu_t  }{  \tilde{R}_t } + \frac{\eta}{2} \Linf{ R - \tR_t}^2 + \frac{1}{\eta} \Big(  D_\Phi(\mu, \mu_t) - D(\mu, \mu_{t+1})  \Big) \nn \\
&= \ip{\mu}{R} + \ip{\mu - \mu_t}{ \tR_t - R}+ \frac{\eta}{2} \Linf{ R - \tR_t}^2 + \frac{1}{\eta} \Big(  D_\Phi(\mu, \mu_t) - D(\mu, \mu_{t+1})  \Big)   \label{eq:hold11}.
\end{align}Taking expectation and summing up \eqref{eq:hold11}, we get
\beq
\sum_{t=1}^T \ip{\mu_{t+1} - \mu}{R} \leq  \frac{1}{\eta}\Big(  D_\Phi(\mu, \mu_1) - D(\mu, \mu_{T+1})  \Big) + \frac{\eta}{2}\sum_{t=1}^T \EE\Linf{ R - \tR_t}^2
\eeq which finishes the proof by dropping the negative term $- D(\mu, \mu_{T+1}) $.
\end{proof}



==> conceptual.tex <==
\SetKwInput{Kw}{Hyperparameters}
\section{Conceptual Algorithms and Their Convergence Rates}
\subsection{Infinite-Dimensional Mirror Descent}
\begin{algorithm} \label{alg:InfMD}
   \caption{\textsc{Inf MD}}
   \KwIn{Initial distributions $\mu_1, \nu_1$}
   %\Kw{s}
   %$\KwOut{$con(r_i)$}
   %$con(r_i)= \Phi$\;
   \For{$t =1, 2, \dots ,T$}
   {
      $\nu_{t+1}=\MD{\nu_t}{-G^\dag \mu_t}, \quad \mu_{t+1}=\MD{\mu_t}{ -g+G\nu_t}$\;
%      $\tnu_{t+1}=\MD{\tnu_t}{-G^\dag \mu_{t}}$\; %\quad \tmu_{t+1}=\MD{\tmu_t}{ -g+G\nu_{t}}$\;
   }
  return $\nu_{t}$'s and $\mu_t$'s.
\end{algorithm}

\subsection{Infinite-Dimensional Mirror-Prox}
\begin{algorithm}\label{alg:InfMP}
   \caption{\textsc{Inf MP}}
   \KwIn{Initial distributions $\tmu_1, \tnu_1$}
   %\Kw{s}
   %$\KwOut{$con(r_i)$}
   %$con(r_i)= \Phi$\;
   \For{$t =1, 2, \dots ,T$}
   {
      $\nu_{t}=\MD{\tnu_t}{-G^\dag \tmu_t}, \quad \mu_{t}=\MD{\tmu_t}{ -g+G\tnu_t}$\;
      $\tnu_{t+1}=\MD{\tnu_t}{-G^\dag \mu_{t}}, \quad \tmu_{t+1}=\MD{\tmu_t}{ -g+G\nu_{t}}$\;
   }
  return $\nu_{t}$'s and $\mu_t$'s.
\end{algorithm}



\begin{algorithm}
   \caption{\textsc{Approx Inf Mirror-Prox}}
   \KwIn{}
   %\Kw{s}
   %$\KwOut{$con(r_i)$}
   %$con(r_i)= \Phi$\;
   \For{$t =1, 2, \dots ,T$}
   {
      $C\leftarrow \tilde{W}[t] \cup \left( \cup_{s=1}^{t-1} W[s] \right), \quad D\leftarrow \tilde{\Theta}[t] \cup \left( \cup_{s=1}^{t-1} \Theta[s] \right)$  \;
     $\vw_t^1 \leftarrow \text{UNIF}(\tilde{W}[t]), \quad \vtheta_t^1 \leftarrow \text{UNIF}(\tilde{\Theta}[t])$\;
      \For{$k=1,2, \dots, K, \dots, K+s$}
      {
         Generate $A=\{X_1, \dots, X_m\} \sim \PP_{\vtheta_t^k}$\;
         $\vtheta_t^{k+1} = \vtheta_t^k + \frac{\gamma \eta}{ms}\nabla_\vtheta \sum_{X_i \in A}\sum_{\vw\in C} f_\vw(X_i) + \sqrt{2\gamma} \Ncal(0,I)  $\;
         Generate $B=\{X'_1, \dots, X'_m\} \sim \PP_{\textup{real}}$\;
         \For{\textup{each} $\vtheta \in D$}
         {
             Generate $\tilde{B}=\{X''_1, \dots, X''_m\} \sim \PP_{\vtheta}$\;
             $B' \leftarrow B'\cup \tilde{B} $\;
         }
          $\vw_t^{k+1} = \vw_t^k + \gamma \eta  \left( \frac{t}{m}\nabla_\vw\sum_{X'_i \in B}  f_{\vw_t^k}(X'_i) - \frac{1}{ms} \nabla_\vw\sum_{X''_i \in B' } f_{\vw_t^k}(X''_i)\right) + \sqrt{2\gamma}\Ncal(0,I)   $\;
      }
      $W[t] \leftarrow\{\vw_t^{K+1} , \dots, \vw_t^{K+s} \}, \quad \Theta[t] \leftarrow \{  \vtheta_t^{K+1}, \dots, \vtheta_t^{K+s}  \}$\;
      \ \\
      $C'\leftarrow  \cup_{s=1}^{t} W[s], \quad D'\leftarrow  \cup_{s=1}^{t} \Theta[s]$  \;
      $\tilde{\vw}_t^1 \leftarrow \text{UNIF}(\tilde{W}[t]), \quad \tilde{\vtheta}_t^1 \leftarrow \text{UNIF}(\tilde{\Theta}[t])\;
      $\;
      \For{$k=1,2, \dots, K, \dots, K+s$}
      {
         Generate $A=\{X_1, \dots, X_m\} \sim \PP_{\tilde{\vtheta}_t^k}$\;
         $\tilde{\vtheta}_t^{k+1} = \tilde{\vtheta}_t^k + \frac{\gamma \eta}{ms}\nabla_\vtheta \sum_{X_i \in A}\sum_{\vw\in C'} f_\vw(X_i) + \sqrt{2\gamma}\Ncal(0,I)    $\;
         Generate $B=\{X'_1, \dots, X'_m\} \sim \PP_{\textup{real}}$\;
         \For{\textup{each} $\vtheta \in D'$}
         {
             Generate $\tilde{B}=\{X''_1, \dots, X''_m\} \sim \PP_{\vtheta}$\;
             $B' \leftarrow B'\cup \tilde{B} $\;
         }
          $\tilde{\vw}_t^{k+1} = \tilde{\vw}_t^k + \gamma \eta  \left( \frac{t}{m}\nabla_\vw\sum_{X'_i \in B}  f_{\tilde{\vw}_t^k}(X'_i) - \frac{1}{ms} \nabla_\vw\sum_{X''_i \in B' } f_{\tilde{\vw}_t^k}(X''_i)\right) + \sqrt{2\gamma} \Ncal(0,I)   $\;
      }
      $\tilde{W}[t] \leftarrow\{\tilde{\vw}_t^{K+1} , \dots, \tilde{\vw}_t^{K+s} \}, \quad \tilde{\Theta}[t] \leftarrow \{  \tilde{\vtheta}_t^{K+1}, \dots, \tilde{\vtheta}_t^{K+s}  \}$\;
   }
  $\texttt{idx}\leftarrow \textup{UNIF}(1, 2, \dots, T)$\;
  return $W[\texttt{idx}], \Theta[\texttt{idx}]$\;
\end{algorithm}
%\section{InfMD}
%\begin{algorithm}
%   \caption{\textsc{InfMD}}
%   \KwIn{Initial point $\vx_1$, Langevin iterations $L$, epochs $M$, learning rate $\eta$, SGLD step-size $\eta'$}
%   %\Kw{s}
%   %$\KwOut{$con(r_i)$}
%   %$con(r_i)= \Phi$\;
%   \For{$m\leq M$}
%   {
%      $\vx \leftarrow \vx_m$\;
%   	  $B' \leftarrow$ sample a mini-batch of size $b$\;
%      $B \leftarrow B \cup B'$\;
%   	  $\vx_m \leftarrow \textup{SGLD}_B(\vx,\eta,L,b)$\;
%   }
%  return $\vx_1, \dots \vx_m$\;
%\end{algorithm}



\subsection{Convergence Rates}


\begin{theorem}[Convergence Rates]\label{thm:convergence_rates}
Let $\Phi$ be the entropic mirror map. Let $M$ be such that $\Linf{-g + G\nu}\leq M$ and $\Linf{G^\dag\mu}\leq M$, $D_0 \coloneqq D(\mu_\star,\mu_1) + D(\nu_\star,\nu_1)$ be the initial distance to the NE. Then
\begin{enumerate}
\item Deterministic gradients, \textbf{Algorithm~\ref{alg:InfMD}} converges at rate $O\left(\frac{1}{\sqrt{T}} \right)$.

\item Stochastic gradients, \textbf{Algorithm~\ref{alg:InfMD}} converges at rate $O\left(\frac{1}{\sqrt{T}} \right)$.

\item Deterministic gradients, \textbf{Algorithm~\ref{alg:InfMP}} converges at rate $O\left(\frac{1}{T} \right)$.

\item Stochastic gradients, \textbf{Algorithm~\ref{alg:InfMP}} converges at rate $O\left(\frac{1}{\sqrt{T}} \right)$.
\end{enumerate}
\end{theorem}

\textbf{Remark:} High probability results can also be obtained as follows: By standard analysis for Stochastic Mirror Descent and Stochastic Mirror-Prox, it suffices to show that the ``gradient estimates'' are sub-Gaussian. Since the gradients correspond to functions in our setting, and since all the functions are assumed to be bounded, the standard Azuma-Hoeffding inequality \citep{boucheron2013concentration} implies that the stochastic gradients are sub-Gaussian.


%\section{From Conceptual to Implementable}
%
%\section{Equivalent Formulations}
%\subsection{Mirror Prox}
%By (\ref{eq:mirror-descent_optimality}), we have, for some constants $C_1, ..., C_t$,
%\begin{align}
%\drm\Phi(\nu_{t}) &= \drm\Phi(\tnu_t)-\eta \left( -G^\dag \tmu_t\right) +C_t  \nn\\
%&=\drm\Phi( \tnu_{t-1}) - \eta \left( -G^\dag \mu_{t-1}\right) - \left( -G^\dag \tmu_t\right) + C_t + C_{t-1} \nn\\
%&= \cdots \nn \\
%&= \drm\Phi(\tnu_1) - \eta \left(   -G^\dag \tmu_t - G^\dag \sum_{s=1}^{t-1} \mu_s  \right)  + \sum_{s=1}^t C_s  . 
%\end{align}
%Similarly, we have, for some other constants $\tilde{C}_1, ..., \tilde{C}_t$,
%\begin{align}
%\drm\Phi (\tnu_{t+1}) &= \drm\Phi ( \tnu_1 ) - \eta \left(  - G^\dag \sum_{s=1}^{t} \mu_s \right) + \sum_{s=1}^t C'_s,  \\
%\drm\Phi (\mu_{t} )&= \drm\Phi (\tmu_1) - \eta \left(  -th + G\tnu_t + G\sum_{s=1}^{t-1}\nu_s   \right)+   \sum_{s=1}^t C''_s,   \\
%\drm\Phi( \tmu_{t+1}) &= \drm\Phi( \tmu_1) - \eta \left(   -th+ G\sum_{s=1}^{t}\nu_s  \right) +\sum_{s=1}^t C'''_s  
%\end{align}for some constants $C'_s, C''_s, C'''_s$'s.
%
%\section{Benefits}
%Parallel computation

